Coding4Games: Can Modern Coding Agents Play Modern Video Games?

Games, especially modern AAA games, challenge language models to perceive complex scenes, control actions, and make decisions over long horizons. Existing game benchmarks primarily test language models as computer-use agents that query a language model throughout play, incurring repeated inference cost and, in real-time games, acting while the environment continues to evolve. We ask whether coding agents can learn from game interaction to develop standalone game-playing programs that run without language model inference. We thus introduce Coding4Games, a benchmark for evaluating whether coding agents can develop standalone programs that play modern games through visual observations and standard game inputs. Coding4Games has three defining features: 1) Diverse Modern Games, covering 15 games with diverse visual, strategic, and control demands; 2) Development-Test Separation, in which a coding agent uses a sandbox and the standard player interface to iteratively develop a program, after which the selected program is frozen and independently tested without language-model inference; and 3) Outcome and Process Evaluation, which measures not only game performance and reliability but also how agents use feedback, revise programs, and resolve problems during development. Across 15 games, the best program per game outscores the strongest GUI baseline on 13 and ties it on one. The human player outscores all agents on 10 games. We additionally examine the effects of development budgets. Coding4Games evaluates whether coding agents can turn their understanding of complex interactive environments into programs that work reliably on their own.

==> Fig/budget_scaling/figures.tex <==
% Checkpoint data from the two supplied workbooks; min--max normalized separately within each curve and panel.
\begin{figure}[t]
\centering
\includegraphics[width=.62\linewidth]{Fig/budget_scaling/fig5_v4.pdf}
\caption{\textbf{Development progress \emph{vs.}\ test performance.} With development capped at 15k game tics and 25M tokens, nonuniformly sampled programs are independently tested for each game. Each row shows the mean test score against game tics and tokens for one game. Axes are rescaled from 0 to 100\% per curve, and stars mark final selected programs.}
\label{fig:tics-performance}
\label{fig:tokens-performance}
\end{figure}


==> Sec/reproducibility_statement.tex <==
% \subsection*{Reproducibility statement}
% The main text and supplementary material describe the benchmark protocol, game tasks, and evaluation procedures. We will release the complete benchmark code, execution and evaluation scripts, and experimental logs when the paper is made publicly available. Reproducing the experiments requires access to the relevant games, a Windows machine, and the model APIs used in our study. A consolidated archive of experimental configurations and setup instructions is not yet available.

